Holomorphic Floer Theory and the Fueter Equation

We outline a proposal for a $2$-category $\mathrm{Fuet}_M$ associated to a hyperk\"ahler manifold $M$, which categorifies the subcategory of the Fukaya category of $M$ generated by complex Lagrangians. Morphisms in this $2$-category are formally the Fukaya--Seidel categories of holomorphic symplectic action functionals. As such, $\mathrm{Fuet}_M$ is based on counting maps to $M$ satisfying the Fueter equation with boundary values on holomorphic Lagrangians. We make the first step towards constructing this category by establishing some basic analytic results about Fueter maps, such as the energy bound and maximum principle. When $M=T^*X$ is the cotangent bundle of a K\"ahler manifold $X$ and $(L_0, L_1)$ are the zero section and the graph of the differential of a holomorphic function $F: X \to \mathbb{C}$, we prove that all Fueter maps correspond to the complex gradient trajectories of $F$ in $X$, which relates our proposal to the Fukaya--Seidel category of $F$. This is a complexification of Floer's theorem on pseudo-holomorphic strips in cotangent bundles. Throughout the paper, we suggest problems and research directions for analysts and geometers that may be interested in the subject.

==> ComplexGradient.tex <==
\section{Complex gradient trajectories}

\subsection{Complex gradient equation}

Let $(X,I,g)$ be an almost Hermitian manifold and let $F \colon X \to \C$ be an $I$-holomorphic function. Its differential $\rd F$ is a complex one-form of type $(1,0)$, so its dual $\overline\nabla F$ with respect to the Riemannian metric is a complex vector field of type $(0,1)$. If $F = f+ig$ with $f$ and $g$ real, then $\nabla g = I\nabla f$ and 
\begin{equation*}
    \overline\nabla F = \nabla f + i \nabla g.
\end{equation*}
% \begin{remark}
%     As a sanity check, we compute 
%     \begin{equation*}
%         i\overline\nabla F = i\nabla f - \nabla g = -i I\nabla g - I\nabla f = -I(\overline\nabla F),
%     \end{equation*}
%     so indeed $\overline\nabla F$ is a vector field of type $(0,1)$.
% \end{remark}
Given a map $u \colon \C \to X$, its differential at every point decomposes into the $I$-linear and $I$-antilinear parts $\del_I u$ and $\delbar_I u$. Since $\delbar_I u$ is an $I$-antilinear map $\C \to TX$, it can be identified with a complex vector of type $(0,1)$. Denoting by $z = s+it$ the coordinate on $\C$, this vector is given by
\begin{equation*}
    \delbar_I u = (\partial_s u + I\partial_t u) + i (I\partial_s u - \partial_t u).
\end{equation*}
The \emph{complex gradient equation} for a map $u \colon \C \to X$ is 
\begin{equation*}
    \delbar_I u = \overline{\nabla} F(u), 
\end{equation*}
or, equivalently,
\begin{equation}
    \label{Eq_ComplexGradient}
    \partial_s u + I(u)\partial_t u = \nabla f(u).
\end{equation}
Since the Cauchy--Riemann operator is conformally invariant, the complex gradient equation has a $\C^*$ symmetry in the following sense. Given $\lambda \in \C^*$, define $u_\lambda(z) = u(\lambda z)$ and $F_\lambda = \bar\lambda F$. Then $u$ is a complex gradient trajectory of $F$ if and only if $u_\lambda$ is a complex gradient trajectory of $F_\lambda$. In particular, if we define a new coordinate on $\C$ by $z_\lambda= s_\lambda + i t_\lambda = \lambda z$, then \eqref{Eq_ComplexGradient} is equivalent to
\begin{equation*}
    \partial_{s_\lambda} u + I(u)\partial_{t_\lambda}u = \nabla \Re(\bar\lambda F). 
\end{equation*}

\subsection{Maximum principle}

\red{
Under what assumptions do we have a maximum principle for complex gradient trajectories?
}

\subsection{Energy bounds}


% \section{Taming Floer's equation}

% Given a complex vector space $(V,I)$ and $v \in V$, a \emph{linear Floer map} is a linear map $u \colon \R^2 \to V$ satisfying
% \begin{equation*}
%     u_s + I(u_t - v) = 0,
% \end{equation*}
% where $(s,t)$ are coordinates on $\R^2$ and $u = (u_s,u_t)$. We say that a triple of forms $\omega\in\Lambda^2 V^*$, $\alpha,\beta \in V^*$ \emph{tames} $(I,v)$ if for every non-zero linear Floer map $A\colon \R^2 \to V$, the following two-form on $\R^2$ is positive:
% \begin{equation*}
%     A^*\omega + \rd s \wedge A^*\alpha  + \rd t \wedge A^*\beta >0.
% \end{equation*}
 

% \begin{lemma}
%   \label{Lem_TamingPair}
%   Let $(V,I)$ be a complex vector space with a Euclidean inner product and let $v \in V$. A triple of forms $(\omega,\alpha,\beta)$ tames $(I,v)$ if and only if there is $c>0$ such that for every linear Floer map $u \colon \R^2 \to V$
%   \begin{equation*}
%       A^*\omega + \rd s \wedge A^*\alpha  + \rd t \wedge A^*\beta  \geq c( |u_s|^2 + |u_t-v|^2) \rd s \wedge \rd t 
%   \end{equation*} 
%   or, equivalently, 
%   if and only if the quadratic function on $V$ given by
%   \begin{equation*}
%       Q(x) = \omega(x,Ix) + \omega(x,v) + \alpha(Ix) - \beta(x) + \alpha(v)   
%   \end{equation*}
%   satisfies
%   \begin{equation*}
%       Q(x) \geq c|x|^2. 
%   \end{equation*} 
% \end{lemma}

% In particular, if $(\omega,\alpha,\beta)$ tames $(I,v)$, then
% \begin{equation*}
%     \omega \text{ tames } I \quad\text{and}\quad \alpha(v) \geq 0,  \quad\text{and}\quad \beta(Iv) < 0.
% \end{equation*} 

% \begin{lemma}
%   If $(\omega,\alpha,\beta)$ tames $(I,v)$ and $\alpha(v)>0$, then $(\omega,\alpha,\beta)$ tames every $(I',v')$ from an open neighborhood of $(I,v)$. 
% \end{lemma}

% We now apply this discussion to Floer's equations on symplectic manifolds. Let $X$ be a manifold equipped with an almost complex structure $I$ and a vector field $V$.  Let 
% \begin{equation*}
%     \omega \in \Omega^2(X) \quad\text{and}\quad \alpha,\beta\in\Omega^1(X)
% \end{equation*}
% be closed forms such that $(\omega,\alpha_1,\alpha_2)$ tames $(I,V)$ at every point of $X$. We consider the Floer equation for maps $u \colon \R^2 \to X$
% \begin{equation*}
%     \partial_s u + I(u)(\partial_t u - V(u)) = 0
% \end{equation*}
% with asymptotic boundary conditions
% \begin{equation*}
%     \lim_{t\to\pm\infty}u(s,t) = x_\pm,
% \end{equation*}
% where $x_\pm$ are zeroes of $V$, and 
% \begin{equation*}
%     \lim_{s\pm\infty} u(s,t) = \gamma_\pm(t),
% \end{equation*}
% where $\gamma_\pm \colon \R \to X$ are integral curves of $V$ from $x_-$ to $x_+$. We assume convergence with derivatives at an exponential rate. Observe that every map $u\colon \R^2 \to X$ with the above asymptotic boundary conditions has a relative homology class 
% \begin{equation*}
%     [u] \in H_2(X,\gamma_-\cup\gamma_+). 
% \end{equation*}
% Equip $X$ with a Riemannian metric compatible with $I$ and define the energy of a map $u \colon \R^2 \to X$ by
% \begin{equation*}
%     E(u) = \int_{\R^2} |\partial_s u|^2 + |\partial_t u - V(u)|^2 
% \end{equation*}

% \begin{lemma}  
%   Suppose that $\omega,\alpha,\beta$ are closed, tame $(I,V)$, and
%   \begin{equation*}
%       \int_{\gamma_\pm} \alpha = 0. 
%   \end{equation*}
%   There is a constant $C>0$ such that for every Floer plane $u \colon \R^2 \to X$ with the asymptotic boundary conditions described above,
%   \begin{equation*}
%       E(u) \leq C \langle [\omega], [u] \rangle.
%   \end{equation*}
% \end{lemma}

==> FukayaSeidelCategory_old.tex <==
\section{Fukaya--Seidel category via Morse theory}

\subsection{Exact Lefschetz fibrations}

\begin{definition}
  \label{Def_LefschetzFibration}
  An exact Lefschetz fibration consists of a manifold with boundary $X$, an exact symplectic form $\omega=\rd\lambda$, an almost complex structure $J$ on $X$ compatible with $\omega$, and a  function $F \colon X \to \C$ satisfying the following:
\begin{itemize}
    \item $F$ is a proper, surjective $J$-holomorphic map,
    \item $F$ has finitely many critical points with distinct critical values, all of which are in the interior of $X$, around every critical point $J$ is integrable, and there is a $J$-holomorphic chart in which
    \begin{equation*}
      F(z_1,\ldots,z_n) = z_1^2 + \ldots + z_n^2.
    \end{equation*}
    \item The boundary of every regular fiber is $J$-convex.
    \item The triple $(F,\omega,J)$ is a locally trivial around infinity the following sense. Let $M$ be a regular fiber of $F$. There is a compact subset $K\subset \C$ such that every point in $\C\setminus K$ has a neighborhood over which $F$ agrees with $M\times\C\to\C$ and $\omega$ and $J$ agree with product symplectic and almost complex structures on $M\times\C$.
    \item The triple $(F,\omega,J)$ is trivial near the boundary in the following sense: $\partial X$ has a neighborhood such that the restriction of $F$ to this neighborhood agrees with the restriction of $M \times \C \to \C$ and $\omega$ and $J$ agree with the product symplectic and almost complex structures on $M\times\C$
\end{itemize}
\end{definition}


The symplectic and almost complex structures induce a Riemannian metric on $X$:
\begin{equation*}
  g(v,w) = \omega(v,Jw).
\end{equation*}

Suppose that the critical values of $F$ are in a convex configuration, that is none of them lies in the convex hull of the others.  After a translation we may assume that zero is a regular value of $F$. Choose an angle $\alpha \in [0,2\pi)$ with the property that no critical value lies on the half-line $\ell_\alpha$ with slope $\alpha$ passing through zero. We will now outline a construction of a directed $A_\infty$ category associated with $\omega$, $J$, $F$, and $\alpha$: 
\begin{equation*}
 \sF = \sF(X,\omega,J,F,\alpha).
\end{equation*} 



\subsection{Objects and morphisms}
The objects of $\sF$ are the critical points of $F$. We order them by the relation
\begin{equation*}
    x \prec y \quad\text{if and only if}\quad \measuredangle(l_\alpha, F(x)) < \measuredangle(l_\alpha, F(y)) ,
\end{equation*}
where $\measuredangle(l_\alpha,F(x))$ is the angle, measured \emph{clockwise}, between $l_\alpha$ and the interval connecting zero with $F(x)$. 
For two critical points $x, y \in \Ob(\sF)$ the morphism group $\Hom(x,y)$ is defined to be trivial if $x \succ y$ and $\Z_2$ if $x=y$. If $x \prec y$, we define $\Hom(x,y)$ to be the $\Z_2$-vector space generated by the gradient trajectories of the functions 
\begin{equation*}
    f_\theta = \Re(e^{-i\theta}F)
\end{equation*}
connecting $x$ and $y$, for all choices of $\theta$. Such a trajectory is a function $\gamma \colon \R\to X$ satisfying  
\begin{gather}
  \label{Eq_GradientFlowline}
    \dot\gamma = \nabla f_\theta(\gamma), \\
    \lim_{t\to-\infty}\gamma(t) = x, \nonumber\\
    \lim_{t\to+\infty}\gamma(t) = y. \nonumber
\end{gather} 

Since $F$ is $J$-holomorphic, the function
\begin{equation*}
    g_\theta = \Im(e^{-i\theta}F)
\end{equation*}
satisfies
\begin{equation}
    \label{Eq_RealImaginaryGradient}
    \nabla g_\theta = J \nabla f_\theta,
\end{equation}
 Therefore, $\nabla f_\theta$ is the Hamiltonian vector field of $g_\theta$ and gradient trajectories of $f_\theta$ are Hamiltonian trajectories of $g_\theta$. In particular, $g_\theta$ is constant along any solution $\gamma$ and the image of $F\circ\gamma$ is contained in 
 \begin{equation*}
      \{ z \in \C : \Im(e^{-i\theta}z) = \mathrm{const} \},
 \end{equation*}  
 which is a line of slope $\theta$.  It follows that for $\gamma$ to exist, $\theta$ must be the slope of the interval  connecting $F(x)$ with $F(y)$. In fact, the image $F\circ\gamma$ is that interval, as shown by the next lemma. We call a tangent vector to $X$ is \emph{horizontal} if it is orthogonal to the fiber of $F$.
 
\begin{lemma}
  \label{Lem_Gradient}
  On $X\setminus\Crit(F)$, the restriction of $F_* \colon TX \to T\C$ to horizontal tangent spaces is conformal with the conformal factor $\rho=\frac12 |\nabla F|^2$. Moreover, $\nabla f_\theta$ is a horizontal vector field and 
  \begin{equation*}
    F_*\nabla f_\theta = \rho \nabla( \Re(e^{-i\theta} z) ).
  \end{equation*}
  In particular, if $\gamma$ is a solution to \eqref{Eq_GradientFlowline}, then $F\circ\gamma$ is a parametrization of the  interval from $F(x)$ to $F(y)$. 
\end{lemma}  
 
\begin{remark}
 The definition of an adapted almost complex structure implies that $\rho=1$ outside a compact subset of the interior of $X$. Therefore, outside such a subset $F$ is a Riemannian submersion. The conformal factor has also a symplectic intepretation as the Poisson bracket $\rho = \{ f_\theta, g_\theta \}$.
\end{remark} 

 Some remarks about the definition of $\Hom(x,y)$ are in order. 

\subsubsection{Compactness}

Let $\sM(x,y)$ be the space of gradient trajectories \eqref{Eq_GradientFlowline} modulo time translations. The fact that every gradient trajectory is mapped under $F$ to the interval connecting $x$ and $y$ together with the triviality of $F$ around $\partial X$ imply that there is a compact subset of $X\setminus\partial X$ containing the image of every trajectory in $\sM(x,y)$. Since there are no critical values on the interval connecting $x$ and $y$,  trajectories cannot break and it follows from standard compactness theory that $\sM(x,y)$ is compact. 


\subsubsection{Linearization}
The linearization of equation \eqref{Eq_GradientFlowline} is the operator
\begin{gather}
  \label{Eq_MorseLinearization}
    \Gamma(\R,\gamma^*TX) \to \Gamma(\R,\gamma^*TX) \nonumber\\
    v \mapsto  \nabla_{\dot\gamma}v - \nabla^2 f_\theta(\gamma)v. 
\end{gather}
where $\nabla^2 f_\theta \colon TX\to TX$ is the Hessian of $f_\theta$. Sections in the $L^2$ kernel of this operator are infinitesimal deformations of $\gamma$. In particular, $\dot\gamma$ is such an infinitesimal deformation, generating time translations of $\gamma$. If the $L^2$ kernel is spanned by $\dot\gamma$, $\gamma$ is an isolated point in $\sM(x,y)$. 

The Hamiltonian interpretation of gradient trajectories provides a different description of the linearization operator.  Hamiltonian trajectories of $g_\theta$ from $x$ to $y$ are critical points of the symplectic action functional on the space of paths $\sP(x,y)$ with exponential convergence to $x$ and $y$ as $t\to \pm\infty$:
\begin{gather}
    \sA_\theta \colon \sP(x,y) \to \R, \nonumber\\
\label{Eq_SymplecticAction}    \sA_\theta(\gamma) = \int_\R \gamma^*\lambda - \int_\R \left[ g_\theta(\gamma(t)) - g_\theta(x)\right] \rd t.
\end{gather}
The second integral is finite by the  exponential convergence. (The integral without the constant term appearing in \cite[Section 2.4]{Haydys2015} and \cite[Section 14.D]{Kontsevich2014} is divergent.) The $L^2$ gradient of $\sA_\theta$ at $\gamma$ is
\begin{equation}
  \label{Eq_GradientOfActionFunctional}
     J(\gamma)\dot\gamma + \nabla g_\theta(\gamma),
\end{equation}
and the Hessian of $\sA_\theta$ at $\gamma$ is the operator 
\begin{gather}
  L_\gamma \colon \Gamma(\R,\gamma^*TX) \to \Gamma(\R,\gamma^*TX), \nonumbering \\
  \label{Eq_Linearization}
L_\gamma v = J(\gamma)\nabla_{\dot\gamma}v + \nabla_v J(\gamma)\dot\gamma + \nabla^2 g_\theta(\gamma)v.
\end{gather}
Differentiating \eqref{Eq_RealImaginaryGradient} shows that if $\gamma$ is a gradient trajectory, then $L_\gamma$ agrees with the linearization operator \eqref{Eq_MorseLinearization}, after multiplying by $J$. The advantage of using $L_\gamma$ is that it is symmetric with respect to the $L^2$ inner product for every $\gamma$;  see  \autoref{Lem_LinearizationIsSymmetric} in \autoref{Sec_SymplecticActionFunctional}.

We say that a  gradient trajectory $\gamma$ is \emph{nondegenerate} if the $L^2$ kernel of $L_\gamma$ is spanned by $\dot\gamma$. If this is true for all trajectories connecting $x$ and $y$, then $\sM(x,y)$ is a discrete space. Together the compactness result discussed earlier, this implies that $\sM(x,y)$ is a finite set. 

\begin{remark}
  The nondegeneracy condition has the following geometric meaning. Denote by $U_x$ and $S_y$ the ascending and descending manifolds of $x$ and $y$ with respect to $f_\theta$; then $\gamma$ is nondegenerate if and only if $U_x$ and $S_y$ intersect cleanly along $\gamma$, that is $TU_x \cap TS_y$ is spanned by $\dot\gamma$. (Note that $U_x$ and $S_y$ cannot intersect transversely because $x$ and $y$ have the same Morse index.)  In other words, $\gamma$ is nondegenerate if and only if the vanishing cycles associated with $x$ and $y$ intersect transversely when transported along the interval connecting $F(x)$ and $F(y)$.  Another equivalent condition is that the family of Morse functions $(f_{\theta+\epsilon})$, as $\epsilon$ varies from negative to positive, satisfies the Morse--Smale condition for families, so that the  continuation map in Morse homology $\HM(f_{\theta-\epsilon}) \to \HM(f_{\theta+\epsilon})$  is given by counting points in $\sM(x,y)$.
\end{remark} 

\subsection{Transversality and tamed Lefschetz fibrations}

In order to ensure that all gradient trajectories are nondegenerate, we might have to perturb the data $(\omega,J,F)$. Since gradient trajectories of $f_\theta$ are Hamiltonian trajectories of $g_\theta$, they depend only on the symplectic structure and not on $J$ and the induced Riemannian metric. Similarly, the nondegeneracy condition for gradient trajectories does not depend $J$. (This is an infinite-dimensional manifestation of the fact that the Hessian of a function at a critical point is independent of the choice of a Riemannian metric.) Therefore, it is necessary to perturb $\omega$ or $F$. In \autoref{Def_LefschetzFibration}, $\omega$ and $F$ are related by requiring that $F$ is $J$-holomorphic with respect to some $J$ which is compatible with $\omega$. This is a closed condition, and it is convenient to replace it by the following open condition.

\begin{definition}
  Let $\omega$ be a symplectic form on $X$ and $F \colon X \to \C$ a smooth function with finitely many complex Morse critical points. We say that the pair $(\omega,F)$ is tamed if $\omega$ tames the standard complex structure in a neighborhood of each critical point and
  \begin{equation*}
      \{ f, g \} > 0,
  \end{equation*}
  where $f = \Re(F)$, $g = \Im(F)$, and $\{\cdot,\cdot\}$ denotes the Poisson bracket with respect to $\omega$.
\end{definition}

This condition can be interpreted in two ways. First, one can show that if $(\omega,F)$ is a  tamed pair, then there exists an almost complex structure $J'$ which is tamed by $\omega$ and has the properties from \autoref{Def_LefschetzFibration}; in particular, $F$ is a $J'$-holomorphic function:
\begin{equation}
    \label{Eq_FJHolomorphic}
    \rd F \circ J' = i\rd F.
\end{equation}
On the other hand, there is another tamed almost complex structure $J$ such that regular fibers of $F$ are $J$-holomorphic and the Hamiltonian vector fields of $f$ and $g$ are related by
\begin{equation}
  \label{Eq_ComplexHamiltonianField}
    X_g = J X_f, 
\end{equation}
or equivalently, the complex vector field $X_f + iX_g$ is of type $(1,0)$. In general, however, $J' \neq J$ since in the tamed case conditions \eqref{Eq_FJHolomorphic} and \eqref{Eq_ComplexHamiltonianField} do not coincide, unlike in the compatible case.

\begin{proposition}
  In the above situation, for every $\theta$, the function $f_\theta$ is Morse and satisfies $\Crit(f_\theta) = \Cirt(F)$, and the vector field $X_{g_\theta}$ is gradient-like for $f_\theta$.
\end{proposition}

\begin{proof}
  First, observe that $X_g$ is gradient-like for $f$, as away from critical points,
  \begin{equation*}
      \rd f(X_g) = \omega(X_f,X_g) = \{ f,g\} >0,
  \end{equation*}
  and similarly $-X_f$ is gradient-like for $g$. Therefore, and since $\rd f(X_f) = \rd g(X_g) = 0$,
  \begin{align*}
      \rd f_\theta (X_{g_\theta}) &= (\cos\theta \rd f + \sin\theta \rd g)(\cos \theta X_g - \sin\theta X_f) \\
      &= \cos^2\theta \rd f(X_g) - \sin^2\theta \rd g(X_f) > 0. \qedhere
  \end{align*}
\end{proof}

\begin{proposition}
   Let $(X,\omega,J,F)$ be an exact Lefschetz fibration. Then $\omega$ can be pertrubed by an arbitrarily small, exact perturbation to a symplectic form $\omega'$ such that the pair $(\omega',F)$ is tamed and all Hamiltonian trajectories of $g_\theta = \Im(e^{-i\theta} F)$ are nondegenerate for every $\theta$.
\end{proposition} 
 
{\color{red} I'm pretty sure that in the tamed case the Morse construction of the Fukaya--Seidel category still works: we have energy bounds and maximum principle for Hamiltonian trajectories and Floer strips.}
 
 
 
We can introduce even more general setup.

\begin{definition}
  Let $(X,\omega)$ be a symplectic manifold and let $F = f+ig$ be a complex-valued function on $X$ with Morse singularities. A pair $(J,V)$ consisting of an almost complex structure and vector field is \emph{tamed} by the pair $(\omega,F)$ if
  \begin{itemize}
     \item in a neighborhood of every critical point, $J$ is integrable, $\omega$ is a K\"ahler form for $J$, and $V=\nabla f$,
      \item $\rd f(V) > 0$, that is $V$ is gradient-like for $f$,
      \item $\rd g(V) = 0$,
      \item for every non-zero tangent vector $\zeta$, 
      \begin{equation*}
          \omega(\zeta,J\zeta) + \omega(\zeta,V) + \rd g(\zeta) > 0.
      \end{equation*}
  \end{itemize}
\end{definition}

These condition imply that: 
\begin{itemize}
    \item there is an a priori energy bound for the integral curves of $V$ connecting given critical points,
    \item $g$ is constant along the integral curves of $V$,
    \item there is an a priori energy bound for solutions of Floer's equation
    \begin{equation*}
        \partial_s u + J(u)(\partial_t u - V(u)) = 0,
    \end{equation*}
    which are asymptotic to integral curves of $u$ as $s\to\pm\infty$ and to critical points of $F$ as $t\to\pm\infty$. 
\end{itemize}


 
 
 
 
\subsubsection{Grading}
\label{sec:grading} For two gradient trajectories $\gamma_0, \gamma_1 \in \Hom(x,y)$ which are homotopic relative endpoints by a homotopy $\Gamma \colon [0,1]\times\R\to X$, we define the relative grading
\begin{equation*}
    \gr(\gamma_0,\gamma_1;\Gamma) \in \Z
\end{equation*}
in the following way. Set $\gamma_s = \Gamma(s,\cdot)$. Parallel transport along the paths $s\mapsto\Gamma(s,\cdot)$, gives us unitary isomorphisms
\begin{equation*}
    \gamma_s^*TX \cong \gamma_0^*TX,
\end{equation*}
so that $L_{\gamma_s}$ can be seen as a family of operators on the same space 
\begin{equation*}
      L_{\gamma_s} \colon \Gamma(\R,\gamma_0^*TX) \to \Gamma(\R,\gamma_0^*TX).
\end{equation*}
These operators are Fredholm when acting on Sobolev completions of the spaces of sections, and they are symmetric with respect to the $L^2$ inner product. The relative grading is defined as the spectral flow of this family
\begin{equation*}
    \gr(\gamma_0,\gamma_1;\Gamma) = \SF( L_{\gamma_s} )_{s\in[0,1]}.
\end{equation*}
Since $L_{\gamma_i}$ has kernel spanned by $\dot\gamma_i$ for $i=0,1$, the spectral flow is defined by shifting the spectrum up to make the endpoints have trivial kernel \cite{Atiyah}.

The relative grading can be interpreted as a relative Maslov index of a path of Lagrangians. By \autoref{Lem_LinearizationIsSymmetric}, every path $\gamma \colon [a,b] \to X$ defines a symplectic isomorphism
\begin{equation*}
  \phi_\gamma \colon T_{\gamma(a)}X \to T_{\gamma(b)}X
\end{equation*}
by solving the ordinary differential equation $L_\gamma v =0$ with prescribed initial value at $t=a$ and evaluating the solution at $t=b$. Choose local trivializations of $TX$ around $x$ and $y$. For every $s\in[0,1]$, we obtain a symplectic isomorphism
\begin{equation*}
    \phi_s \colon T_x X \to T_y X
\end{equation*}
by composing the isomorphism $T_{\gamma_s(-t)} X \to T_{\gamma_s(t)}X$ for $t$ very large, with the isomorphisms $T_{\gamma_s(-t)} X \cong T_x X$ and $T_{\gamma_s(t)} X \cong T_y X$  given by the local trivializations. At $x$ and $y$ we have distinguished Lagrangian subspaces
\begin{equation*}
    \Delta_x \subset T_x X \quad\text{and}\quad \Delta_y \subset T_y X
\end{equation*}
given by the negative eigenspaces of the Hessian $\nabla^2 f_\theta$. (We use here that $f_\theta$ is the real part of a $J$-holomorphic function and $J$ is integrable around critical points.) Thus, the familt $(\gamma_s)_{s\in[0,1]}$ defines a path of pair of Lagrangians in $T_y X$
\begin{equation*}
    (\phi_s(\Delta_x), \Delta_y) 
\end{equation*}
and the relative grading is the relative Maslov index of this path:
\begin{equation*}
    \gr(\gamma_0,\gamma_1;\Gamma) = \mu(\phi_s(\Delta_x),\Delta_y).
\end{equation*}

The relative grading can be upgraded to absolute grading if $2c_1(X,\omega) = 0$ in $H^2(X,\Z)$, as explained in \cite{Seidel}. If this is the case, the bundle of Lagrangian Grassmanians $\sL(TX) \to X$ can has a fiberwise universal cover $\widetilde\sL(TX) \to X$. Choose a lift $\widetilde\Delta_x$ of $\Delta_x$ at every critical point. For every gradient trajectory $\gamma \in \Hom(x,y)$ the Lagrangian subspace $\phi_\gamma(\Delta_x)$ has a lift $\phi_\gamma(\widetilde\Delta_x)$ obtained by transporting $\widetilde\Delta_x$ along $\gamma$. 
The absolute grading $\gr(\gamma)$ is then defined as the Maslov index 
of the loop of Lagrangians  in $T_y X$ obtained by composing the canonical short path from $\phi_\gamma(\Delta_x)$ to $\Delta_y$ with the image of a path from $\widetilde\Delta_y$ to  $\phi_\gamma(\widetilde\Delta_x)$ under the covering map $\widetilde\sL(T_y X) \to \sL(T_y X)$. For any homotopy $\Gamma$ between two gradient trajectories $\gamma_0$ and $\gamma_1$, we have
\begin{equation*}
    \gr(\gamma_0, \gamma_1; \Gamma) = \gr(\gamma_1) - \gr(\gamma_0).
\end{equation*}


\subsection{$A_\infty$-operations}
For critical points $x_0 \prec x_1 \prec \ldots \prec x_n$, the higher product
\begin{equation*}
    m_n \colon \Hom(x_0,x_1) \otimes \cdots \otimes \Hom(x_{n-1}, x_n) \to \Hom(x_0,x_n) 
\end{equation*}
is defined by counting solutions to the Floer equation asymptotic to gradient trajectories. We begin by outlining the construction of
\begin{equation*}
    m_1 \colon \Hom(x_0,x_1) \to \Hom(x_0,x_1).
\end{equation*}
This map is the differential of the Floer complex associated with the symplectic action functional  \eqref{Eq_SymplecticAction} on the space of paths  $\sP(x_0,x_1)$. Here $\theta = \theta(x_0,x_1)$ is the slope of the line from $F(x_0)$ to $F(x_1)$. 
Given a gradient trajectory $\gamma_0 \in \Hom(x_0,x_1)$, define
\begin{equation*}
    m_1(\gamma_0) = \sum_{\gamma_1 \in \Hom(x_0,x_1)} N(\gamma_0;\gamma_1) \gamma_1,
\end{equation*}
where $N(\gamma_0;\gamma_1)$ is the mod $2$ count of solutions to the Floer equation
\begin{gather}
    u \colon \R^2 \to X, \nonumber\\
  \label{Eq_FloerEquation}
  \partial_s u + J(u)(\partial_t u - \nabla f_{\theta}(u)) = 0,
\end{gather}
with asymptotic boundary conditions
\begin{gather}
   \label{Eq_BoundaryConditions}
    \lim_{s\to-\infty} u(s,\cdot) = \gamma_0, \quad
    \lim_{s\to+\infty} u(s,\cdot) = \gamma_1, \\
    \lim_{t\to-\infty} u(\cdot,t) = x_0, \quad
    \lim_{t\to+\infty} u(\cdot, t) = x_1,  \nonumber
\end{gather}
and finite energy
\begin{equation}
  \label{Eq_FloerEnergy}
    E (u) =  \frac12 \int_{\R^2} |\partial_s u|^2 + |\partial_t u - \nabla f_\theta (u)|^2  < \infty.
\end{equation}

The $n$-th higher operation is defined similarly, by counting solutions to   \label{Eq_FloerEquation} with $n+1$ boundary conditions. The starting point is the observation that Floer's equation \eqref{Eq_FloerEquation} for $\theta=0$, can be written as
\begin{equation}
  \label{Eq_WittenEq}
    \delbar_J(u) + \Im( \overline{\nabla F}(u) \otimes_\C \rd\bar z ) = 0.
\end{equation}
where $z=s+it$ is the holomorphic coordinate on $\C=\R^2$, and
\begin{align*}
    \delbar_J(u) &=   \rd u + J(u) \circ \rd u \circ i   \\
    &=   (\partial_s u + J(u)\partial_t u) \otimes \rd s + (\partial_t u - J(u)\partial_s u) \otimes \rd t  
\end{align*}
is the $J$-antilinear part of the $\rd u$, while
\begin{equation*}
   \overline{\nabla F} =   \nabla f - i\nabla g 
\end{equation*}
is the complex vector field on $X$ dual to the $(1,0)$ form $\rd F = \del_J F$. 

\begin{remark}
  We follow here the symplectic geometry convention which interprets $\delbar_J(u)$ as a section of $J$-antilinear maps $T\C \to u^*TX$. It complex geometry  it is more common to interpret $\delbar_J(u)$ as a section of $T^{0,1}\C \otimes_\C u^*TX$, with complex structure on $TX$ given by $J$:
  \begin{equation*}
      \delbar_J(u) =  (\partial_s u + J \partial_t u) \otimes_\C \rd\bar z. 
  \end{equation*}
  Similarly, using the complex isomorphism between $T_{1,0}X \subset TX\otimes\C$ and $(TX,J)$, we can identify the complex vector field $\overline\nabla F$ a section of $TX$. With respect to these identification, Floer's equation has the form
  \begin{equation*}
      \delbar_J(u) + \overline{\nabla F}(u) \otimes_\C \rd\bar z = 0,
  \end{equation*}
  which is the equation appearing in \cite{gaiotto-moore-witten}, \cite{Kontsevich2014}.
\end{remark}
 
Unlike the Cauchy--Riemann equations, \eqref{Eq_WittenEq} is not conformally invariant. In particular, after the holomorphic change of coordinates $z' = e^{i\theta}z$, \eqref{Eq_WittenEq} reads
\begin{equation*}
    \delbar_J(u) + \Im(  \overline{\nabla e^{-i\theta} F}\otimes_\C \rd\bar z' ) = 0,
\end{equation*}
or, in real coordinates $z' = s' + it'$,
\begin{equation*}
    \partial_{s'}u + J(u)(\partial_{t'}u - \nabla f_{\theta}(u) ) = 0.
\end{equation*}
This suggests that it is possible for a finite energy solution to converge to a gradient trajectory of $f_0$ as $t \pm \infty$ and to a gradient trajectory of $f_\theta$ as $t' \to \pm\infty$. More generally, we expect that there are solutions which in different regions of the plane are asymptotic to gradient trajectories of $f_\theta$ for \emph{different} values of $\theta$. 

We can now give a putative definition of the $A_\infty$ operations on $\sF$. Given $\gamma_i \in \Hom(x_i,x_{i+1})$ for $i=0,\ldots, n-1$, define
\begin{equation}
  \label{Eq_AInftyOperation}
    m_n(\gamma_0\otimes\cdots\otimes\gamma_{n-1}) = \sum_{\gamma_n\in\Hom(x_0,x_n)} N(\gamma_0,\ldots\gamma_{n-1};\gamma_n) \gamma_n,
\end{equation}
where the coefficient $N(\gamma_0,\ldots\gamma_{n-1};\gamma_n)$ is defined by counting solutions to Floer's equation \eqref{Eq_WittenEq} with the following asymptotic conditions. Let $\theta_i$ be the slope of the interval from $F(x_i)$ to $F(x_{i+1})$, and introduce the holomorphic coordinate 
\begin{equation*}
    z_k = s_k + it_k =  e^{i\theta_k}z.
\end{equation*}
For $k=0,\ldots, n-1$, we require that as $s_i \to -\infty$, the restriction $u(s_i,\cdot)$ converges to the gradient trajectory $\gamma_i$ of $f_{\theta_i}$. For $i=n$, we require convergence to $\gamma_n$ as $s_n\to +\infty$. In  defining $ N(\gamma_0,\ldots\gamma_{n-1};\gamma_n)$ we should specify a finite energy condition similar to \eqref{Eq_FloerEnergy}, but stating a precise energy condition and asymptotic at infinity is a nontrivial task. 

\subsubsection{Compactness}

Let  $\sM(\gamma_0,\ldots \gamma_{n-1};\gamma_n)$ be the moduli space of solutions to \eqref{Eq_WittenEq} asymptotic to $\gamma_0,\ldots,\gamma_{n-1}$ in the negative ends ant to $\gamma_n$ in the positive end.  A basic difficulty in defining \eqref{Eq_AInftyOperation} is proving a compactness result for $\sM(\gamma_0,\ldots \gamma_{n-1};\gamma_n)$. The first step is to show that all solutions stay within a fixed compact subset of the interior of $X$.

\begin{proposition}[Maximum principle]
 Let $F \colon X \to \C$ be an exact Lefschetz fibration equipped with an adapted almost complex structure $J$. Let $\Sigma$ be a compact Riemann surface with boundary and let $\zeta$ be an antiholomorphic $(0,1)$-form on $\Sigma$. There exists a compact subset $K \subset X \setminus \partial X$ with the following property. If $u \colon \Sigma \to X$ is a solution to Floer's equation
  \begin{equation*}
      \delbar_J(u) + \Im(\overline{\nabla F}(u) \otimes_\C\zeta) = 0
  \end{equation*}
  such that $u(\partial \Sigma) \subset K$, then $u(\Sigma) \subset K$.
\end{proposition}

\begin{proof}
  Since $J$ is adapted to $F$, there exists $R>0$ such that $|\nabla F|$ is constant on the set $\{ |F| > R \}$.  Set $v = F\circ u$. We will show that if $|v| \leq R$ on $\partial \Sigma$, then $|v| \leq R$ on $\Sigma$. Suppose, by contradiction, that $|v|$ attains its maximum at a point $z \in \Sigma\setminus\partial\Sigma$ such that $|v(z)|>R$. 
  It follows from Floer's equation that $v$ satisfies
  \begin{equation*}
    \delbar v = i | \nabla F(u) |^2 \zeta.
  \end{equation*}
  Since $|\nabla F(u)|$ is constant in a neighborhood of $z$, in that neighborhood
  \begin{equation*}
      \Delta v = 4\del \delbar v = 4\del( i|\nabla F(u)|^2 \zeta) = \mathrm{constant} \cdot \del \zeta = 0,
  \end{equation*}
  so $v$ is harmonic, which is a contradiction with the maximum modulus principle since $|v|$ attains maximum at $z$. 
  In a neighborhood of the boundary, $X$ is symplectomorphic to the product of $\partial M\times(-\epsilon,0]$ with $\C$, where $M$ is a regular fiber of $F$, and $F$ agrees with the trivial fibration. In that region, $u= (u_0,v)$ where $u_0$ is a map into $\partial M\times(-\epsilon,0]$. Floer's equation implies that $u_0$ is $J$-holomorphic. Since $\partial M$ is $J$-convex,  the standard argument using maximum principle shows that $u_0(\Sigma)$ is contained in the interior of $M$ unless it intersects $\partial M$. 
\end{proof} 
 
The next step is establishing an a priori energy bound for solutions to Floer's equation. For solutions with two asymptotic ends  such a bound follows from the standard energy identity in Floer theory. 
 
\begin{proposition}[Energy identity]
  \label{Prop_FloerEnergyIdentity}
  The energy \eqref{Eq_FloerEnergy} of every solution $u \colon \R^2 \to X$ to Floer's equation \eqref{Eq_Floer} with asymptotic boundary conditions \eqref{Eq_BoundaryConditions} is 
  \begin{equation*}
      E(u) = \int_{\gamma_1}\lambda - \int_{\gamma_0}\lambda
  \end{equation*}
\end{proposition}
\begin{proof}
  Let $S,T>0$ and $\Sigma  = [-S,S]\times[T,T]$. By the energy identity for Floer's trajectories (\autoref{Prop_EnergyIdentity} applied to the Hamiltonian perturbation $\cH = -H \rd t$), 
  \begin{equation*}
      E(u|_{\Sigma}) = \int_\Sigma u^*\omega + \int_{\partial\Sigma} (H\circ u) \rd t, 
  \end{equation*}
  where $H = g_\theta - g_\theta(x_0)$ is the Hamiltonian. Therefore,
  \begin{equation*}
       E(u|_{\Sigma}) = \int_{\partial\Sigma} u^*\lambda  + \int_{-T}^T H(u(S,t))\rd t - \int_{-T}^T H(u(-S,t)) \rd t. 
  \end{equation*}
  Since $H\circ\gamma_0 = H\circ\gamma_1 = 0$, in the limit $S\to\infty$ the right-hand side converges to
  \begin{equation*}
     \int_{-T}^T (\gamma_1)^*\lambda - \int_{-T}^T (\gamma_0)^*\lambda 
  \end{equation*}
  and the result follows by taking the limit $T \to \infty$. 
\end{proof}

The situation is more complicated for solutions with more than two asymptotic ends. Given a solution asymptotic to gradient trajectories of $f_{\theta_0}, \ldots, f_{\theta_n}$, in the $k$th asymptotic end with coordinate $z_k = e^{i\theta_k}z$ we want to control \eqref{Eq_FloerEnergy} for $\theta=\theta_k$. The difficulty is that the integrand of \eqref{Eq_FloerEnergy} is not preserved under the change of coordinates $z \to z_k$, that is:
\begin{equation*}
    |\partial_{s_k} u|^2 + |\partial_{t_k}u-\nabla f_{\theta_k}(u)|^2 \neq |\partial_{s_l} u|^2 + |\partial_{t_l}u-\nabla f_{\theta_l}(u)|^2 \quad\text{for } k \neq l.
\end{equation*}
Another possible notion of energy is
\begin{equation*}
    E_\cH(u) = \int |\rd u - X_\cH(u)|^2
\end{equation*}
where $\cH = \Im(F \rd\bar z)$ is the Hamiltonian-valued one-form which leads to equation \eqref{Eq_WittenEq}. Now the integrand remains unchanged if $z$ is replaced by $e^{i\theta}z$ and $F$ by $e^{-i\theta}F$. However, as pointed out in \cite{gaiotto-moore-witten}, this energy is infinite for any solution $u$ asymptotic to gradient trajectories $\gamma_0,\ldots,\gamma_n$. Namely, if $Q_\Lambda \subset \C$ is a square whose sides have length $\Lambda$, then  
 \begin{equation*}
     E_{\cH}(u|_{Q_\Lambda}) +  \int_{Q_\Lambda}|\nabla F(u)|^2 =  \int_{Q_\Lambda} u^*\omega  +  ( |F(z_+)-F(z_-)| )\Lambda + o(\Lambda). 
 \end{equation*}
It is an interesting problem to find the right notion of energy which is globally defined and has an a priori bound for solutions asymptotic to gradient trajectories of $f_\theta$ for different angles $\theta$. Given the right notion of energy, one should prove that the ends of the moduli space  $\sM(\gamma_0,\ldots \gamma_{n-1};\gamma_n)$ are given by the usual phenomenon of breaking of Floer polygons. We expect that this leads to the $A_\infty$ relations for $m_1,m_2,\ldots$.  \cite{xx} suggest that this is true only under the assumption that the critical values $F(x_0), \ldots, F(x_n)$ are in a convex position. If this is not the case and there is another critical value in the convex hull of $F(x_0), \ldots, F(x_n)$ we expect an additional noncompactness phenomenon given by breaking Floer polygons into subpolygons with vertex on the interior critical value. 
 
\iffalse 
For $z' = e^{i\theta}z$,
\begin{align*}
    s' &= \cos\theta s - \sin\theta t, \\
    t' &= \sin\theta s + \cos\theta t. 
\end{align*}
and
\begin{align*}
    \partial_s u &= \cos\theta \partial_{s'}u + \sin\theta\partial_{t'}u, \\
    \partial_t u &= -\sin\theta \partial_{s'}u + \cos\theta \partial_{t'}u. 
\end{align*}
If $u$ satisfies
\begin{equation*}
    \partial_s u + J (\partial_t u - \nabla f) =0,
\end{equation*}
then it satisfies
\begin{equation*}
    \partial_{s'}u + J(\partial_{t'}u - \nabla f_\theta) = 0,
\end{equation*}
where 
\begin{equation*}
    f_\theta = \Re(e^{-i\theta} F) = \cos\theta f + \sin\theta g.
\end{equation*}
Rewriting the energy in the $z'$ coordinate,
\begin{align*}
     |\partial_s u|^2 + |\partial_t u - \nabla f|^2 &= |\partial_s u|^2 + |\partial_t u|^2 - 2\langle \partial_t u, \nabla f \rangle + |\nabla f|^2 \\
    &= |\partial_{s'}u|^2 + |\partial_{t'}u|^2 - 2\langle  -\sin\theta \partial_{s'}u + \cos\theta \partial_{t'}u, \nabla f\rangle + |\nabla f_\theta|^2 \\ 
    &= |\partial_{s'}u|^2 + |\partial_{t'}u|^2 - 2\langle \partial_{t'} u, \cos\theta\nabla f + \sin\theta\nabla g\rangle +  |\nabla f_\theta|^2 \\
     &  \qquad\qquad\qquad + 2\sin\theta \{ \langle \partial_{s'}u,  \nabla f\rangle +  \langle \partial_{t'}u,  \nabla g\rangle \} \\
     &= |\partial_{s'}u|^2 + |\partial_{t'}u - \nabla f_\theta|^2 + 2\sin\theta\langle \partial_{s'}u-J\partial_{t'}u, \nabla f\rangle. 
\end{align*}
\fi

\subsubsection{Linearization and transversality} 
\begin{itemize}
  \item Fredholm setup for Floer strips
  \item How do we perturb so that moduli spaces are smooth
\end{itemize}



\subsection{Relation to the Fukaya--Seidel category}
In this section we outline the relationship between this construction of the Fukaya-Seidel category and the more traditional constructions \cite{seidel-vanishing-cycles} \cite{seidel-fukaya-categories-and-picard-lefshetz-theory}, and clarify the role of the convexity assumption. 

\red{Write $m$ for the number of critical points of $F$. Write $Crit(F)$ for the critical points of $F$, and $V(F) = F(Crit(F))$ for the critical values.}

    Let $D$ be a disk containing all the critical points of $F$, and let $b_\alpha \in \partial D$ be the intersection of the half-line $l_\alpha$ with $D$. Then we make an \emph{admissible choice of paths} in the sense of \cite[Section~2c]{seidel-vanishing-cycles}: we choose paths $c_1, \ldots, c_{m}$ from $b_\alpha$ to $x_i$, where $i$ is the $i$-th critical point in \red{clockwise} order, as in Figure \ref{fig:fukaya-seidel-comparison-admissible-paths}: namely, the paths do not intersect, enter the convex hull of the critical values of $F$ through the face between $x_1$ and $x_m$, and such that the order by the clockwise tangent vector to $b_\alpha$ agrees with the order of their endpoints. This is sufficient data \red{(modulo definitions of a Lefshetz fibration?)} to define the Fukaya Seidel-category. The vanishing cycles of $\{c_i\}$ are then Lagrangian spheres $\Gamma= (L_1, \ldots, L_{m}$ in $X_{b_\alpha}$, forming a \emph{Lagrangian configuration} as in \cite[Definition~2.1]{seidel-vanishing-cycles}. 
    
    If we have chosen a grading on $X$ and the critical points as in Section \ref{sec:grading}, then we have (by parallel transport) lifts of tangent fibers of the Lefshetz thimbles associated to the paths to $\tilde{\mathcal{L}}(TX)$, and thus a grading of the $\tilde{L}_i$.\red{(does this need comment?)} Then $\tilde{\Gamma} = \{\tilde{L}_i\}$ form a \emph{graded Lagrangian configuration} as in \cite[Section~6a]{seidel-vanishing-cycles}, and we can associated a quasi-isomorphism class of directed $A_\infty$ categories $Lag^\to(\tilde{\Gamma})$. We have the following 
    \begin{conjecture}
    \label{conj:fukaya-seidel-comparison}
    \begin{equation}
    \mathcal{F} \simeq Lag^{\to}(\tilde{\Gamma}).
    \end{equation}
    \end{conjecture}.
    On the level of objects, this equivalence should send $x_i$ to $\tilde{L}_i$. The relation on the level of morphisms can be motivated by the fact that for any pair $1 \leq i< j \leq m$, the triple $(b_\alpha, c_i, c_j)$ is isotopic through triples of points $b_t$ on $\C \setminus V(F)$ and paths $c_i^t, c_j^t$ from $x_i$ and $x_j$ to $b$, to a triple $(b_{ij}, c'_i, c'_j)$ where $b_{ij}$ lies on the straight line from $x_i$ to $x_j$ and $(c'_i, c'_j)$ are the straight-line paths. Trivializing the fiber bundle $X_{b_t}$ along the path $b_t$ in such an isotopy, the vanishing cycles associated to ($c^t_i, c^t_j)$) undergo a Hamiltonian isotopy, so their Floer homology groups are unchanged; thus, have have quasi-isomorphisms of morphism complexes. \red{worth explaining why our Homs really are just Floer homs on the chain level above; otherwise, edit.} Comparing the compositions is a more challenging problem, but it is natural to try to implement the proposal of \cite{gaiotto-moore-witten}, \cite{Kontsevich2014} \red{cite section} in this setting. 

\begin{figure}
\label{fig:fukaya-seidel-comparison-admissible-paths}
	\centering
    \includegraphics[width=0.4\textwidth]{"figures/fukaya-seidel-comparison-admissible-paths.pdf"}
	\caption{Admssible paths to compare with Fukaya-seidel category.}
\end{figure}
	
\subsection{Exact triangles associated to deformations of $F$}

Choose a subset of three critical points $x_1, x_2, x_3$ of $F$, ordered clockwise, and suppose $0 \in Conv(\{x_1, x_2, x_3\})$. We can ask what we happens if we deform $F$ such that the critical value $F(x_2)$ passes through the line between $F(x_1)$ and $F(x_3)$ (Figure \ref{}). In this case, on the level of morphism spaces, parametrized Morse theory (or, alternatively, Picard-Lefshetz theory) shows that 
\[ Hom dimensoins.\]
This suggests that there should exist an exact sequence of groups 
\begin{equation}
    \label{eq:crossing-exact-triangle}
\end{equation}
We expect that such an exact triangle can be proven directly by bifurcation analysis of the associated paramterized $J$-holomorphic curve equations. 

Assuming Conjecture \ref{conj:fukaya-seidel-comparison}, such an exact triangle is also expected to hold. It is a result of Seidel that the derived category $D^b(Lag^\to(\tilde{\Gamma})$ is an invariant of the Lefshetz fibration $F$, and does not depend on the paths $\{c_i\}$ chosen. In particular, (assuming we have chosen a grading on the critical points), every path $\gamma$ from $b_\alpha$ to a critical point and gives rise to an object $\tilde{L}_\gamma \in D^b(Lag^\to(\tilde{\Gamma})$, and the objects associated to paths related by Hurwitz moves are themselves related by mutations: specifically,  ... 
\begin{equation}
    \label{eq:hurwitz-exact-triangle}
    ...
\end{equation}

In fact,  $D^b(Lag^\to(\tilde{\Gamma})$ is an invariant not of $F$ but of a certain deformation class of Lefshetz fibrations $F$.
\begin{lemma}
\label{lemma:deformation-lefshetz-fibration}
Deformation statement.
\end{lemma}


Suppose we are in the minimal case where $\{x_1, x_2, x_3\} = Crit(F)$. Then both $\{x_1, x_2, x_3\}$ and $\{x'_1, x'_2, x'_3\}$ are in convex position; applying Conjecture \ref{conj:fukaya-seidel-comparison}, we get that ...

\subsection{Non-convex case and invariance}
The algebraic definition of $\mathcal{F}$ given in this paper is only expected to be correct in the case where $V(F)$ lie in general convex position. For the non-convex case,  there are physical \cite{gaiotto-moore-witten} (when $F$ is strictly holomorphic) and mathematical \cite{Kontsevich2014} proposals for how to define the correct category. Intuitively, one reason why the non-convex case is distinct from the convex case is that in the non-convex case, \emph{there does not exist an equivalence class of paths $\{c_i\}$ from the critical points to the basepoints $b_\alpha$ which can be deformed to paths arising from the straight-line paths}; see Figure \ref{}. 

We expect that a modification of the analysis in this paper can adapt the ideas of \cite{Kontsevich2014} to define $\mathcal{F}$ in the setting where there is no convexity condition on $V(F)$, in which case 
(need to explain why we automatically get the derived category) $\mathcal{F} \simeq D^\pi\mathcal{F} \simeq Tw Lag^\to(\tilde{\Gamma})$. 


==> SymplecticActionFunctional.tex <==
\section{Symplectic action functional}
\label{Sec_SymplecticActionFunctional}

Let $(X,\omega)$ be a symplectic manifold. Given a function $H \colon X \to \R$, the Hamiltonian vector field is given by
\begin{equation*}
  \omega(\cdot,X_H) = \rd H.
\end{equation*}
The equation for a map $\gamma \colon \R \to X$ to be a Hamiltonian trajectory is
\begin{equation*}
    \dot\gamma = X_H(\gamma).
\end{equation*}
Choose a compatible almost complex structure $J$ and denote by $\nabla$ the Levi--Civita connection of the Riemannian metric
\begin{equation*}
    \langle v,w\rangle = \omega(v,Jw).
\end{equation*}
Using the metric, we can write the Hamiltonian trajectory equation equivalently as
\begin{equation*}
    J(\gamma)\dot\gamma + \nabla H(\gamma) = 0.
\end{equation*}
The left-hand side is the gradient of the symplectic action functional with respect to the $L^2$ metric on the space of paths. 
The linearization of the last equation is  
\begin{gather*}
    L_\gamma \colon \Gamma(\R,\gamma^*TX) \to \Gamma(\R,\gamma^*TX) \\
    L_\gamma v = J(\gamma)\nabla_{\dot\gamma}v + \nabla_v J(\gamma)\dot\gamma + \nabla^2 H(\gamma) v.
\end{gather*}
Here $\nabla_{\dot\gamma}$ denotes the covariant derivative in the direction of the vector field $\partial/\partial t$ with respect to the connection on $\gamma^*TX$ pulled back from $\nabla$. At points where $\dot\gamma \neq 0$, it agrees with the covariant derivative in the direction of $\dot\gamma$ in  $X$.

The operator $L_\gamma$ is the Hessian of the symplectic action functional with respect to the $L^2$ metric. 

\begin{lemma} \label{Lem_LinearizationIsSymmetric}
  For all $\gamma \colon [a,b]\to X$ and $v,w \in \Gamma([a,b],\gamma^*TX)$, we have
  \begin{equation*}
    \int_a^b \langle L_\gamma v, w \rangle   - \langle v, L_\gamma w \rangle  = \omega(v(b),w(b)) - \omega(v(a),w(a)).
  \end{equation*} 
  In particular, 
  \begin{itemize}
    \item if $L_\gamma v = L_\gamma w = 0$, then $\omega(v,w)$ is a constant function on $[a,b]$;
    \item if $[a,b]=\R$ and $v$ and $w$ converge to zero at $\pm\infty$, then
        \begin{equation*}
      \langle L_\gamma v, w \rangle_{L^2} = \langle v, L_\gamma w \rangle_{L^2},
  \end{equation*} 
  and $L_\gamma$ is an unbounded symmetric operator on $L^2(\R,\gamma^*TX)$ with dense domain $W^{1,2}(\R,\gamma^*TX)$.
  \end{itemize}
\end{lemma}

\begin{proof}
  Writing $J = J(\gamma)$, and so forth, we compute
  \begin{align*}
      &\langle L_\gamma v, w \rangle  - \langle v, L_\gamma w \rangle & \\
      &= \underbrace{\langle J\nabla_{\dot\gamma} v, w \rangle  - \langle v, J\nabla_{\dot\gamma} w \rangle}_{(1)}  
      + \underbrace{\langle \nabla_v J \dot\gamma, w \rangle - \langle v, \nabla_w J \dot\gamma \rangle}_{(2)}  
      + \underbrace{\langle \nabla^2H v, w \rangle - \langle v, \nabla^2H w \rangle}_{(3)}. 
  \end{align*}
  The third term vanishes since $\nabla^2 H$ is symmetric. Integrating by by parts yields
  \begin{equation*}
   \int_a^b (1) = \int_a^b \frac{\rd}{\rd t} \langle Jv, w \rangle +  \langle v , \nabla_{\dot\gamma} J w \rangle 
  \end{equation*}
  Therefore,
  \begin{equation*}
      \int_a^b (1) + (2) = \omega(v(b),w(b)) - \omega(v(a),w(a)) + 
      \int_a^b \langle v , \nabla_{\dot\gamma} J w \rangle + \langle \nabla_v J \dot\gamma, w \rangle - \langle v, \nabla_w J \dot\gamma \rangle.  
  \end{equation*}
  The integral on the right-hand side vanishes by virtue of the identities
  \begin{gather*}
     \langle \nabla_u J v, w \rangle + \langle \nabla_v J w, u \rangle + \langle \nabla_w J u, v \rangle = \rd\omega(u,v,w) = 0, \\
     \langle \nabla_u J v , w \rangle + \langle v , \nabla_u J w \rangle = 0,
  \end{gather*}
  which are consequences of $\langle \cdot, \cdot \rangle = \omega(\cdot, J\cdot)$ and the fact that $\nabla$ preserves the metric; see \cite[Lemma C.7.1]{McDuff2012}.
\end{proof}

\begin{corollary}
  Every path $\gamma \colon [a,b] \to \R$  defines a symplectic isomorphism
  \begin{equation*}
      \phi_\gamma \colon T_{\gamma(a)} X \to T_{\gamma(b)} X
  \end{equation*}
  by 
  \begin{equation*}
      \phi_\gamma v = \tilde v(b),
  \end{equation*}
  where $\tilde v \in \Gamma([a,b], \gamma^*TX)$ is the unique solution of the initial value problem
  \begin{equation*}
      L_\gamma \tilde v = 0, \quad \tilde v(a) = v.
  \end{equation*}
\end{corollary}
